A Distributed Online Pricing Strategy for Demand Response Programs

We study a demand response problem from utility (also referred to as operator)'s perspective with realistic settings, in which the utility faces uncertainty and limited communication. Specifically, the utility does not know the cost function of consumers and cannot have multiple rounds of information exchange with consumers. We formulate an optimization problem for the utility to minimize its operational cost considering time-varying demand response targets and responses of consumers. We develop a joint online learning and pricing algorithm. In each time slot, the utility sends out a price signal to all consumers and estimates the cost functions of consumers based on their noisy responses. We measure the performance of our algorithm using regret analysis and show that our online algorithm achieves logarithmic regret with respect to the operating horizon. In addition, our algorithm employs linear regression to estimate the aggregate response of consumers, making it easy to implement in practice. Simulation experiments validate the theoretic results and show that the performance gap between our algorithm and the offline optimality decays quickly.

==> offline_new.tex <==
%change structure as follows:
% 1. introduce the problem that why we do not know the information. why this scenario is more realistic
% 2. Say what metric we use the evaluate the algorithm. why use regret, what are the components to compute regret
% 3. State the main theorem. (case 2 as another minor theorem and its proof is left to appendix). The proof of the main theorem is left to section III.
% 4. State the optimal solution with full information (centralized scheduling)

%\input{main_results}



If both $\alpha_i$ and $\beta_i$ are known to the utility, then it suffices to solve the optimization problem in \eqref{case1_formulation} and \eqref{case2_formulation} and the utility will obtain the optimal scheduling of each user. Note that the constraint $x^t_i \geq 0$ naturally follows from the structure of the formulation, therefore there are no explicit inequality constraints in problem \eqref{case1_formulation}.

It is, however, more common that $\alpha_i$ and $\beta_i$ are some unknown parameters from users that the utility does not know in advance. Therefore, it is impossible for the utility to solve the problem in  \eqref{case1_formulation} and  \eqref{case2_formulation} directly. We therefore target distributed algorithms that allow utilities to send signals to users in order to learn the parameters and at the same time solve the problem as accurately as possible.

Since Case 1 adopts an easier form of the cost function (as is a special case of Case 2 when $\alpha_i = 0$), we first consider Case 1 as an illustrating example and then extend the discussion to Case 2.

\subsection{Optimal solution for Case 1}
We determine the optimal value of $Y$, which is the capacity of the demand reduction prior to the operation of demand response program in each time slot. To do this, we consider $Y$ as a parameter and $\mathbf{Q}, \mathbf{x}_i$ as decision variables in the optimization problem \eqref{case1_formulation}. The optimal solution for $\mathbf{Q}, \mathbf{x}_i$ as a function of $Y$ can be obtained by Lagragian relaxation. Then plug in these solutions into the objective function in \eqref{case1_formulation} . Since there is no constraint on $Y$, we simply take the derivative of the objective function respect to $Y$ equal to zero, which yields the optimal $Y^*$ as:
\begin{equation}\label{Ystar1}
Y^* = \frac{T\alpha(1+\sum_i \frac{1}{\beta_i})}{\sum_t d_t^2}
\end{equation}

Given $Y^*$, we need to solve the following problem that derives the optimal demand response of all the users $i \in \mathcal{N}$ over time slots $t \in \mathcal{T}$:
\begin{equation}\label{formulation_new}
\begin{aligned}
& \min_{\mathbf{Q}, \{\mathbf{x}_i,\forall i \in \mathcal{N}\} } && \sum_{t\in\mathcal{T}} \left[ \sum_{i\in\mathcal{N}} \frac{1}{2 N} \beta_i (x_i^{t})^2 + \frac{1}{2N} (Q_t - Y^* d_t)^2 \right] \\ %- \frac{\alpha Y^* T}{N}
& \text{subject to}
&& Q_t- \sum_{i\in\mathcal{N}} x_i^t = 0 \\
& \text{variables:}
&&\{ Q_t, x_i^t, ~i \in \mathcal{N},~t\in\mathcal{T} \}.
\end{aligned}
\end{equation}

Note that here $x_i^t \geq 0$ is omitted because it is always satisfied.

To solve the problem in \eqref{formulation_new}, we relax the equality constraint 
$Q_t- \sum_{i\in\mathcal{N}} x_i^t = 0$ with a dual variable $\lambda_t$ and it is easy to see that the \eqref{formulation_new} can be decomposed exactly in the form of \eqref{user_optimization} where the price signals are replaced by dual variables $\lambda_t$. This decomposition technique by Lagrangian relaxation is commonly used in Unit Commitment (UC) problems [cite papers XXX].


By Lagrandian relaxation, we obtain the optimal solution to \eqref{formulation_new} as:
\begin{equation}\label{optimal1}
\begin{aligned}
& \lambda_{t}^{*} = \frac{Y^* d_t}{N+ \sum_{i\in\mathcal{N}} \frac{N}{\beta_i}} \\
& x_{i}^{t,*} =  \frac{N \lambda_t^*}{\beta_i}  = \frac{N Y^* d_t}{\beta_i \left( \sum_{i\in\mathcal{N}}\frac{N}{\beta_i} + N \right)}
\end{aligned}
\end{equation}

If we are able to observe noiseless responses $x_{i}^{t}$, then with one arbitrary initial $\lambda_0$, we are able to determine the parameters $\beta_i$ in just one round. However, it is more realistic to consider a noisy setting, where users exhibit noisy responses to price signals. In this case, it is impossible to recover the values of $\beta_i$ after just one price signal. Therefore it is crucial to come up with an online strategy that assigns price signals optimally so that the demand reduction from the users do not deviate too much from the goal, meanwhile the values of $\beta_i$ can be recovered as accurately as possible.

Specifically, in a noisy setting, user $i$'s response under a given reward signal $\lambda_t$ (generated from any algorithm) is shown as
\begin{equation}\label{optimal1_noise}
 \hat{x}_{i}^{t} = \hat{x}_{i}^{t} (\lambda_t) = \frac{N \lambda_t}{\beta_i} + \epsilon_i^t,
\end{equation}
which contains white noise $\epsilon_i^t$ (i.i.d. standard Gaussian noise), and the aggregated demand reduction is denoted as $\hat{Q}_t = \sum_{i \in \mathcal{N}} \hat{x}_{i}^{t}$.



\subsection{Optimal solution for Case 2}
A more general case is when $\alpha_i \neq 0$. Similarly, we first determine the optimal value of $Y$ as
\begin{equation}\label{Ystar2}
Y^* = \frac{T\alpha(1+\sum_i \frac{1}{\beta_i})^2 - \sum_t (\sum_i \frac{\alpha_i}{\beta_i})(1+ \sum_i \frac{1}{\beta_i})d_t}{\sum_t d_t^2 (1+\sum_i \frac{1}{\beta_i})}
\end{equation}

As long as $\alpha$ is big enough, we can ensure that $Y^* = \Theta (N)$.

Given $Y^*$, we need to solve the following problem to derive the optimal demand response of all the users $i \in \mathcal{N}$ over time slots $t \in \mathcal{T}$:

\begin{comment}
	\begin{equation}\label{complete}
	\begin{aligned}
	& \min_{\mathbf{Q}, \{\mathbf{x}_i,\forall i \in \mathcal{N}\} } && \sum_{t\in\mathcal{T}} \sum_{i\in\mathcal{N}} \frac{1}{N} \left( \frac{1}{2} \beta_i (x_i^{t})^2 + \alpha_i x_i^{t} \right) \\
	&&& + \sum_{t\in\mathcal{T}}  \frac{1}{2N} (Q_t - Y^* d_t)^2 \\ %- \frac{\alpha Y^* T}{N}
	& \text{subject to}
	&& Q_t- \sum_{i\in\mathcal{N}} x_i^t = 0 \\
	&&& x_i^t \geq 0 \\
	& \text{variables:}
	&&\{ Q_t, x_i^t, ~i \in \mathcal{N},~t\in\mathcal{T} \}.
	\end{aligned}
	\end{equation}
	
\end{comment}

\begin{equation}\label{simplified}
\begin{aligned}
& \min_{\mathbf{Q}, \{\mathbf{x}_i,\forall i \in \mathcal{N}\} } && \sum_{t\in\mathcal{T}}  \sum_{i\in\mathcal{N}} \frac{1}{N} \left( \frac{1}{2} \beta_i (x_i^{t})^2 + \alpha_i x_i^{t} \right) \\
&&&+ \sum_{t\in\mathcal{T}} \frac{1}{2N} (Q_t - Y^* d_t)^2 \\ %- \frac{\alpha Y^* T}{N}
& \text{subject to}
&& Q_t- \sum_{i\in\mathcal{N}} x_i^t = 0 \\
& \text{variables:}
&&\{ Q_t, x_i^t, ~i \in \mathcal{N},~t\in\mathcal{T} \}.
\end{aligned}
\end{equation}

Note that in \eqref{simplified}, it is not true that $x_i^t$ is always non-negative. We therefore interpret a positive $x_i^t$ as a reduction in consumption and a negative $x_i^t$ as an increase in consumption. Imposing $x_i^t \geq 0$ will naturally rule out participation of some users (users whose remain dormant in consumption reduction when the price signal is below their thresholds) in the demand response program. This structure is very different from the linear response of users that we discuss in this work and is thus left as future work.

We solve Problem \eqref{simplified} similarly to the discussion in Case 1 using Lagrangian relaxation and obtain the optimal solution as:
\begin{align} \label{optimal2}
& x_{i}^{t,*} = \frac{N \lambda_t^* - \alpha_i}{\beta_i}, \\
& \lambda_{t}^{*} = \frac{Y^* d_t + \sum_{i\in\mathcal{N}} \frac{\alpha_i}{\beta_i} }{N+ \sum_{i\in\mathcal{N}} \frac{N}{\beta_i}}.
\end{align}
where $\lambda_{t}^{*}$ is the optimal value of the dual variable associated with the equality constraint in \eqref{simplified}.

Similarly, it is trivial to consider the noiseless setting as the learning process is done after one observation. Thus we assume that the utility only observes noisy responses from users, and user $i$'s response under a given reward signal $\lambda_t$ is shown as
\begin{equation} \label{optimal2_noise}
  \hat{x}_{i}^{t} = \hat{x}_{i}^{t} (\lambda_t) = \frac{N \lambda_t^* - \alpha_i}{\beta_i} + \epsilon_i^t,
\end{equation}
which contains white noise $\epsilon_i^t$, and the aggregated demand reduction is denoted as $\hat{Q}_t = \sum_{i \in \mathcal{N}} \hat{x}_{i}^{t}$.

